Stochastic Neighbor Embedding under f-divergences

The t-distributed Stochastic Neighbor Embedding (t-SNE) is a powerful and popular method for visualizing high-dimensional data. It minimizes the Kullback-Leibler (KL) divergence between the original and embedded data distributions. In this work, we propose extending this method to other f-divergences. We analytically and empirically evaluate the types of latent structure-manifold, cluster, and hierarchical-that are well-captured using both the original KL-divergence as well as the proposed f-divergence generalization, and find that different divergences perform better for different types of structure. A common concern with $t$-SNE criterion is that it is optimized using gradient descent, and can become stuck in poor local minima. We propose optimizing the f-divergence based loss criteria by minimizing a variational bound. This typically performs better than optimizing the primal form, and our experiments show that it can improve upon the embedding results obtained from the original $t$-SNE criterion as well.

==> approx.tex <==
\section{Approximation algorithm for the least squares problem}
\label{sec:approx}

In this section, we consider the least squares problem from \Cref{eq:mle}.
The inputs are an arbitrary matrix $\vX = [ \vx_1 | \vx_2 | \dotsb | \vx_n ]^\T
\in \R^{n \times d}$ and an arbitrary vector $\vy = (y_1,y_2,\dotsc,y_n)^\T \in
\R^n$, and the goal is to find a vector $\vw \in \R^d$ and permutation matrix
$\vPi \in \cP_n$
(where $\cP_n$ denotes the space of $n \times n$ permutation matrices\footnote{%
  Each permutation matrix $\vPi \in \cP_n$ corresponds to a permutation $\pi$ on
  $[n]$; the $(i,j)$-th entry of $\vPi$ is one if $\pi(i) = j$ and is zero
  otherwise.%
}) to minimize $\norm[0]{\vX\vw - \vPi^\T\vy}_2^2$.
This problem is NP-hard in the case where $d = \Omega(n)$
\citep{pananjady2016linear} (see also \Cref{sec:npc}).
We give an approximation scheme that, for any $\epsilon \in \intoo{0,1}$,
returns a $(1+\epsilon)$-approximation in time $(n/\epsilon)^{O(k)} +
\poly(n,d)$, where $k := \rank(\vX) \leq \min\{n,d\}$.

We assume without loss of generality that $\vX \in \R^{n \times k}$ and $\vX^\T
\vX = \vI_k$.
This is because we can always replace $\vX$ with its matrix of left singular
vectors $\vU \in \R^{n \times k}$, obtained via singular value decomposition
$\vX = \vU \vvarSigma \vV^\T$, where $\vU^\T\vU = \vV^\T\vV = \vI_k$ and
$\vvarSigma \succ 0$ is diagonal.
A solution $(\vw,\vPi)$ for $(\vU,\vy)$ has the same cost as the solution
$(\vV\vvarSigma^{-1}\vw,\vPi)$ for $(\vX,\vy)$,
and a solution $(\vw,\vPi)$ for $(\vX,\vy)$ has the same cost as the solution
$(\vvarSigma\vV^\T\vw,\vPi)$ for $(\vU,\vy)$.

\subsection{Algorithm}

\begin{algorithm}[t]
  \renewcommand\algorithmicrequire{\textbf{input}}
  \renewcommand\algorithmicensure{\textbf{output}}
  \caption{Approximation algorithm for least squares problem}
  \label{alg:approx}
  \begin{algorithmic}[1]
    \REQUIRE
    Covariate matrix $\vX = [ \vx_1 | \vx_2 | \dotsb | \vx_n ]^\T \in \R^{n
    \times k}$;
    response vector $\vy = (y_1,y_2,\dotsc,y_n)^\T \in \R^n$;
    approximation parameter $\epsilon \in \intoo{0,1}$.

    \renewcommand\algorithmicrequire{\textbf{assume}}
    \REQUIRE
    $\vX^\T\vX = \vI_k$.

    \ENSURE
    Weight vector $\hat{\vw} \in \R^k$ and permutation matrix $\hat{\vPi} \in
    \cP_n$.

    \STATE
    Run ``Row Sampling'' algorithm with input matrix $\vX$ to obtain a matrix
    $\vS \in \R^{r \times n}$ with $r = 4k$.

    \STATE
    Let $\cB$ be the set of vectors $\vb = (b_1,b_2,\dotsc,b_n)^\T
    \in \R^n$ satisfying the following: for each $i \in [n]$,
    \begin{itemize}[leftmargin=2em]
      \item
        if the $i$-th column of $\vS$ is all zeros, then $b_i = 0$;

      \item
        otherwise, $b_i \in \cbr[0]{ y_1, y_2, \dotsc, y_n}$.

    \end{itemize}

    \STATE Let $c := 1+4(1 + \sqrt{n/(4k)})^2$.

    \FOR{each $\vb \in \cB$}

      \STATE
      Compute $\tilde\vw_{\vb} \in \argmin_{\vw \in \R^k} \norm[0]{\vS(\vX\vw -
      \vb)}_2^2$, and let $r_{\vb} := \min_{\vPi \in \cP_n}
      \norm[0]{\vX\tilde\vw_{\vb} - \vPi^\T\vy}_2^2$.

      \STATE
      Construct a $\sqrt{\epsilon r_{\vb}/c}$-net $\cN_{\vb}$ for the Euclidean
      ball of radius $\sqrt{cr_{\vb}}$ around $\tilde\vw_{\vb}$, so that for
      each $\vv \in \R^k$ with $\norm[0]{\vv - \tilde\vw_{\vb}}_2 \leq
      \sqrt{cr_{\vb}}$, there exists $\vv' \in \cN_{\vb}$ such that
      $\norm[0]{\vv - \vv'}_2 \leq \sqrt{\epsilon r_{\vb}/c}$.

    \ENDFOR

    \RETURN
    $\displaystyle\hat\vw \in \argmin_{\vw \in \bigcup_{\vb \in \cB} \cN_{\vb}}
    \min_{\vPi \in \cP_n} \norm[0]{\vX\vw - \vPi^\T\vy}_2^2$
    and
    $\displaystyle\hat\vPi \in \argmin_{\vPi \in \cP_n} \norm[0]{\vX\hat\vw -
    \vPi^\T\vy}_2^2$.

  \end{algorithmic}
\end{algorithm}

Our approximation algorithm, shown as \Cref{alg:approx}, uses a careful
enumeration to beat the na\"ive brute-force running time of $\Omega(|\cP_n|) =
\Omega(n!)$.
It uses as a subroutine a ``Row Sampling'' algorithm of
\citet{boutsidis2013near} (described in \Cref{sec:approx-details}), which has
the following property.

\begin{theorem}[Specialization of Theorem 12 in \citep{boutsidis2013near}]
  \label{thm:row-sampling}
  There is an algorithm (``Row Sampling'') that, given any matrix $\vA \in \R^{n
  \times k}$ with $n\geq k$, returns in $\poly(n,k)$ time a matrix $\vS \in
  \R^{r \times n}$ with $r = 4k$ such that the following hold.
  \begin{enumerate}[leftmargin=2em,itemsep=0ex]
    \item
      Every row of $\vS$ has at most one non-zero entry.

    \item
      For every $\vb \in \R^n$, every $\vw' \in \argmin_{\vw \in \R^k}
      \norm[0]{\vS(\vA\vw - \vb)}_2^2$ satisfies $\norm[0]{\vA\vw' - \vb}_2^2
      \leq c \cdot \min_{\vw \in \R^k} \norm[0]{\vA\vw - \vb}_2^2$ for $c = 1 +
      4(1+\sqrt{n/(4k)})^2 = O(n/k)$.

  \end{enumerate}
\end{theorem}

The matrix $\vS$ returned by Row Sampling determines a (weighted) subset of
$O(k)$ rows of $\vA$ such that solving a (ordinary) least squares problem (with
any right-hand side $\vb$) on this subset of rows and corresponding right-hand
side entries yields a $O(n/k)$-approximation to the least squares problem over
all rows and right-hand side entries.
Row Sampling does not directly apply to our problem because (1) it does not
minimize over permutations of the right-hand side, and (2) the approximation
factor is too large.
However, we are able to use it to narrow the search space in our problem.

An alternative to Row Sampling is to simply enumerate all subsets of $k$ rows of
$\vX$.
This is justified by a recent result of~\citet{derezinski2017unbiased}, which
shows that for any right-hand side $\vb \in \R^n$, using ``volume
sampling''~\citep{avron2013faster} to choose a matrix $\vS \in \cbr[0]{0,1}^{k
\times k}$ (where each row has one non-zero entry) gives a similar guarantee as
that of Row Sampling, except with the $O(n/k)$ factor replaced by $k+1$ in
expectation.

\subsection{Analysis}

The approximation guarantee of \Cref{alg:approx} is given in the following
\namecref{thm:approx}.

\begin{theorem}
  \label{thm:approx}
  \Cref{alg:approx} returns $\hat{\vw} \in \R^k$ and $\hat{\vPi} \in \cP_n$
  satisfying
  \begin{equation*}
    \norm{\vX\hat{\vw} - \hat\vPi^\T\vy}_2^2
    \ \leq \ (1+\epsilon) \min_{\vw
    \in \R^k, \vPi \in \cP_n} \norm{\vX\vw - \vPi^\T\vy}_2^2
    \,.
  \end{equation*}
\end{theorem}

\begin{proof}
  Let $\opt := \min_{\vw,\vPi} \norm[0]{\vX\vw - \vPi^\T\vy}_2^2$ be the optimal
  cost, and let $(\vw_\star,\vPi_\star)$ denote a solution achieving this cost.
  The optimality implies that $\vw_\star$ satisfies the normal equations
  $\vX^\T\vX\vw_\star = \vX^\T\vPi_\star^\T\vy$.
  Observe that there exists a vector $\vb_\star \in \cB$ satisfying
  $\vS\vb_\star = \vS\vPi_\star^\T\vy$.
  By \Cref{thm:row-sampling} and the normal equations, the vector
  $\tilde{\vw}_{\vb_\star}$ and cost value $r_{\vb_\star}$ satisfy
  \begin{equation*}
    \opt
    \ \leq \
    r_{\vb_\star}
    \ \leq \
    \norm{\vX\tilde{\vw}_{\vb_\star} - \vPi_\star^\T\vy}_2^2
    \ = \
    \norm{\vX(\tilde{\vw}_{\vb_\star} - \vw_\star)}_2^2
    + \opt
    \ \leq \ c \cdot \opt \,.
  \end{equation*}
  Moreover, since $\vX^\T\vX = \vI_k$, we have that
  $\norm[0]{\tilde{\vw}_{\vb_\star} - \vw_\star}_2 \leq \sqrt{(c-1)\opt} \leq
  \sqrt{c r_{\vb_\star}}$.
  By construction of $\cN_{\vb_\star}$, there exists $\vw \in \cN_{\vb_\star}$
  satisfying $\norm[0]{\vw - \vw_\star}_2^2 = \norm[0]{\vX(\vw - \vw_\star)}_2^2
  \leq \epsilon r_{\vb_\star} / c \leq \epsilon \opt$.
  For this $\vw$, the normal equations imply
  \begin{equation*}
    \min_{\vPi \in \cP_n} \norm[0]{\vX\vw - \vPi^\T\vy}_2^2
    \ \leq \
    \norm[0]{\vX\vw - \vPi_\star^\T\vy}_2^2
    \ = \ \norm[0]{\vX(\vw - \vw_\star)}_2^2 + \opt
    \ \leq \ (1+\epsilon) \opt
    \,.
  \end{equation*}
  Therefore, the solution returned by \Cref{alg:approx} has cost no more than
  $(1+\epsilon) \opt$.
\end{proof}

By the results of \citet{pananjady2016linear} for maximum likelihood estimation,
our algorithm enjoys recovery guarantees for $\bar{\vw}$ and $\bar{\pi}$ when
the data come from the Gaussian measurement model~\eqref{eq:measurements}.
However, the approximation guarantee also holds for worst-case inputs without
generative assumptions.

\paragraph{Running time.}

We now consider the running time of \Cref{alg:approx}.
There is the initial cost for singular value decomposition (as discussed at the
beginning of the section), and also for ``Row Sampling''; both of these take
$\poly(n,d)$ time.
For the rest of the algorithm, we need to consider the size of $\cB$ and the
size of the net $\cN_{\vb}$ for each $\vb \in \cB$.
First, we have $|\cB| \leq n^r = n^{O(k)}$, since $\vS$ has only $4k$ rows and
each row has at most a single non-zero entry.
Next, for each $\vb \in \cB$, we construct the $\delta$-net $\cN_{\vb}$ (for
$\delta := \sqrt{\epsilon r_{\vb}/c}$) by constructing a $\delta/\sqrt{k}$-net
for the $\ell_\infty$-ball of radius $\sqrt{cr_{\vb}}$ centered at
$\tilde{\vw}_{\vb}$ (using an appropriate axis-aligned grid).
This has size $|\cN_{\vb}| \leq (4c^2k/\epsilon)^{k/2} = (n/\epsilon)^{O(k)}$.
Finally, each $\argmin_{\vw \in \R^k}$ computation takes $O(nk^2)$ time, and
each $(\arg)\min_{\vPi \in \cP_n}$ takes $O(nk + n \log n)$
time~\citep{pananjady2016linear} (also see \Cref{sec:approx-details}).
So, the overall running time is $(n/\epsilon)^{O(k)} + \poly(n,d)$.


